On the Complexity of Exploration in Goal-Driven Navigation

Building agents that can explore their environments intelligently is a challenging open problem. In this paper, we make a step towards understanding how a hierarchical design of the agent's policy can affect its exploration capabilities. First, we design EscapeRoom environments, where the agent must figure out how to navigate to the exit by accomplishing a number of intermediate tasks (\emph{subgoals}), such as finding keys or opening doors. Our environments are procedurally generated and vary in complexity, which can be controlled by the number of subgoals and relationships between them. Next, we propose to measure the complexity of each environment by constructing dependency graphs between the goals and analytically computing \emph{hitting times} of a random walk in the graph. We empirically evaluate Proximal Policy Optimization (PPO) with sparse and shaped rewards, a variation of policy sketches, and a hierarchical version of PPO (called HiPPO) akin to h-DQN. We show that analytically estimated \emph{hitting time} in goal dependency graphs is an informative metric of the environment complexity. We conjecture that the result should hold for environments other than navigation. Finally, we show that solving environments beyond certain level of complexity requires hierarchical approaches.

==> figures/hippo-algo.tex <==
\begin{algorithm}[t]
\caption{HiPPO (Hierarchical PPO)}
\label{alg:hippo}
\begin{algorithmic}
   \STATE {\bfseries Input:} Meta-controller policy $\pi_M$, Controller policy $\pi_C$
   \FOR{$i=1$ {\bfseries to} num\_episodes}
    \STATE subgoal $g \gets \pi_M(s)$
    \WHILE{$s$ is not terminal}
        \STATE $F \gets 0$
        \STATE $s_0 \gets s$
        \WHILE{{\bfseries not} ($s$ is terminal or $g$ is reached)}
            \STATE action $a \gets \pi_C(\{s, g\})$
            \STATE state $s'$, reward $f \gets \textrm{Environment}(a)$
            \STATE intrinsic reward $r \gets \textrm{Critic}(s', g)$
            \STATE PPO\_Update($\pi_C, s, a, s', r)$
            \STATE $F \gets F + f$
            \STATE $s \gets s'$
        \ENDWHILE
        \STATE PPO\_Update($\pi_M, s_0, g, s', F$)
        \STATE subgoal $g \gets \pi_M(s)$
    \ENDWHILE
   \ENDFOR
\end{algorithmic}
\end{algorithm}



==> figures/mdp.tex <==
\begin{figure}
    \flushleft
    \begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, node distance=1cm, thick,main/.style={circle,draw}, x=1.25cm, y=1.7cm]
        \node[main, fill=gray!30, draw=black!50, label={[label distance=0.15cm]above:terminal}, scale=0.75] (A0) at (0,-2) {0};
        \node[main, fill=white!30, draw=black!50, label={[label distance=0.15cm]above:initial}, scale=0.75] (A1) at (1.1,-2) {1};
        \foreach \i [evaluate=\i as \x using \i*1.1] in {2,...,4} {
            \node[main, fill=white!30, draw=black!50, scale=0.75] (A\i) at (\x,-2) {\i};
        }
        \node[main, fill=yellow!30, draw=black!50, scale=0.75] (A5) at (5.5,-2) {5};
        % Forward arrows
        \foreach \i [count=\j, evaluate=\i as \x using \i*1.1+0.55] in {0,...,4} {
            \draw[nice_red] (A\i) to[out=35,in=145] (A\j);
            \node[circle, draw=none, fill=white, scale=0.5, rotate=-1] (al\i) at (\x, -1.82) {\fontsize{9}{9}\selectfont\textcolor{nice_red}{0.5}};
        }
        \foreach \i [count=\j, evaluate=\i as \x using \i*1.1+0.65] in {0,...,4} {
            \draw[nice_red] (A\j) to (A\i);
            \node[draw=none, fill=white, scale=0.5, rotate=-1] (al\i) at (\x, -2) {\fontsize{9}{9}\selectfont\textcolor{nice_red}{0.5}};
        }
        % Backward arrows
        \foreach \i [count=\j, evaluate=\i as \x using \i*1.1+0.58] in {0,...,4} {
            \draw[nice_blue] (A\j) to[out=-145,in=-35] (A\i);
            \node[draw=none, fill=white, scale=0.5, rotate=-1] (al\i) at (\x, -2.18) {\fontsize{9}{9}\selectfont\textcolor{nice_blue}{1.0}};
        }
    \end{tikzpicture}
    \begin{center}\begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, node distance=1cm, thick,main/.style={circle,draw}, x=1.25cm, y=1.7cm]
        % Legend
        \node (lb1) at (0.3, -2.5) {};
        \node (lb2) at (-0.4, -2.5) {};
        \draw[nice_blue] (lb1) to (lb2);
        \node[draw=none] (blue_arrow) at (0.9, -2.5) {left action};
        \node (lr1) at (1.7, -2.5) {};
        \node (lr2) at (2.4, -2.5) {};
        \draw[nice_red] (lr1) to (lr2);
        \node[draw=none] (red_arrow) at (3.1, -2.5) {right action};
    \end{tikzpicture}\end{center}
    \caption{In the stochastic MDP environment, there are 6 possible states $\{0, 1, \ldots, 5 \}$, and the agent always starts at state 1. The \emph{left} action moves the agent to the left deterministically, but the \emph{right} action has a 50-50 chance of moving the agent right or left. If the agent goes to state 0, the episode terminates and the agent receives either a reward of +1 if it has visited state 5, or a reward of +0.01 otherwise.}
    \label{fig:env-mdp}
\end{figure}

==> sections/scratchwork.tex <==
%!TEX root = ../main.tex

\section{Scratchwork}

\subsection{Environments and Tasks}

\begin{itemize}
    \item Objects: keys, ball, door (4 different colors each).
    \item \textbf{Minigrid 1}: master goal: pickup the right object. [the object is unknown or specified by the goal.]
    \item \textbf{Minigrid 2}: master goal: open the door; sub-goal: (1) pickup the right key. (= taxi driver env in MAXQ) [again, the key and the door are either unknown or specified by the goal.]
    \item \textbf{Minigrid 3}: master goal: pickup an object; sub-goals: (1) pickup the key, (2) open the door.
    \item Representation of the sub-goal: one-hot encoding of the color and the object class.
\end{itemize}

\newpage
\section{Project Roadmap (beyond the workshop)}
The following are approaches roughly ordered by complexity (from plain RL to HRL):
\begin{enumerate}
    \item \textbf{Baselines} (must provide additional information to ensure fair comparison):
    \begin{itemize}
        \item Decompose the task into subgoals. Provide reward for achieving each subgoal.
        \item Provide reward in a hierarchical form to the baselines.
    \end{itemize}
    \item \textbf{Modular policies} (similar to Jacob Andreas’s work):
    \begin{itemize}
        \item Decompose the task into subgoals. Represent subgoals via embeddings.
        \item Train the policy by conditioning on the subgoals. Reward the agent only for solving the task.
        \item Instead of conditioning, could try using separate policy networks for each task and switch between them based on the goal.
    \end{itemize}
    \item \textbf{Modular policies + hierarchical rewards} (?):
    \begin{itemize}
        \item An integration of (1) and (2) -- provide each conditional/modular policy additional rewards for achieving the corresponding subgoals.
    \end{itemize}
    \item \textbf{Hierarchical policies}:
    \begin{itemize}
        \item Train a meta-controller that selects a goal (from a predefined set of goals) for the low-level controller to condition on (similar to Kulkarni et al., 2016).
        \item Alternatively, train a meta-controller that selects a low-level controller (i.e., an option) for the given goal (similar to Bacon et al., 2017). Both the meta-controller and all low-level controllers are trainable.
        \item The controller is rewarded by the meta-controller. Reward is based on whether the goal was attained.
    \end{itemize}
    \item \textbf{Hierarchical policies with learned rewards}:
    \begin{itemize}
        \item Same as (4), but the meta-controller also learns to reward the low-level controller(s). The idea is to also discover better reward so that low-level controller(s) can improve much faster.
    \end{itemize}

    \item \textbf{Goal-discovery}:
    \begin{itemize}
        \item Meta-controller learns to discover goals. Initially, every state is a goal. The meta-controller must learn to select “interesting” and “valuable” states as goals.
        \item Learning relationships between the goals.
    \end{itemize}
\end{enumerate}

==> tables/laplacian-table.tex <==
\begin{table}[]
\centering
\caption{%
Depth, width, and hitting time (HT) statistics computed for \texttt{EscapeRoom} environments (a)-(g)  from Table~\ref{tab:env-escaperoom}.}\label{tab:laplacian}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
                    & (a) & (b) & (c) & (d) & (e) & (f) & (g) \\
\midrule
exit depth          &  2  &  2  &  4  &  2  &  2  &  4  &  6  \\
graph width         &  1  &  2  &  1  &  2  &  3  &  2  &  1  \\
HT (w/o drop-key)   &  8.4 & 12.1 & 15.1 & 13.1 & 13.9 & 29.2 & 27.5  \\
HT (w/ drop-key)     &  16.5 & 25.2 & 39.5 & 27.5 & 26.7 & 86.1 & 82.5  \\
\bottomrule
\end{tabular}
\vspace{-2ex}
\end{table}


==> tables/performance-tables.tex <==
\begin{table}[ht]
\centering
\caption{Average success rate (\%) to reach the final goal over the last 10 training episodes.}\label{tab:success_rate}
\small
\setlength{\tabcolsep}{5.7pt}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
 & (a) & (b) & (c) & (d) & (e) & (f) & (g) \\
\midrule
PPO & 56.1 & 28.2 & 0.2 & 22.7 & 19.1 & 0.0 & 0.0 \\
PPO+Bonus & 9.0 & 6.0 & 0.0 & 11.0 & 4.5 & 0.5 & 0.0 \\
PPO+Sketch & 23.2 & 14.5 & 0.4 & 12.6 & 10.7 & 0.1 & 0.0 \\
HiPPO & \textbf{74.9} & \textbf{57.0} & \textbf{60.8} & \textbf{48.0} & \textbf{29.9} & \textbf{11.2} & \textbf{19.0} \\
\bottomrule
\end{tabular}
\caption{Average episode length (\% of the max length, smaller is more efficient) over the last 10 training episodes.
``--'' indicates that the method failed to reach the final goal within 1000 time steps.}\label{tab:episode-length}
\small
\setlength{\tabcolsep}{5.6pt}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
 & (a) & (b) & (c) & (d) & (e) & (f) & (g) \\
\midrule
PPO & 78.5 & 88.0 & -- & 90.7 & 91.4 & -- & -- \\
PPO+Bonus & 97.8 & 96.7 & 99.9 & 97.3 & 98.0 & 99.9 & -- \\
PPO+Sketch & 91.9 & 94.4 & 99.9 & 95.0 & 95.7 & -- & -- \\
HiPPO & \textbf{48.2} & \textbf{67.4} & \textbf{69.1} & \textbf{71.0} & \textbf{85.3} & \textbf{96.4} & \textbf{93.8} \\
\bottomrule
\end{tabular}
\end{table}

